Aero-Nef: Neural Fields for Rapid Aircraft Aerodynamics Simulations

This paper presents a methodology to learn surrogate models of steady state fluid dynamics simulations on meshed domains, based on Implicit Neural Representations (INRs). The proposed models can be applied directly to unstructured domains for different flow conditions, handle non-parametric 3D geometric variations, and generalize to unseen shapes at test time. The coordinate-based formulation naturally leads to robustness with respect to discretization, allowing an excellent trade-off between computational cost (memory footprint and training time) and accuracy. The method is demonstrated on two industrially relevant applications: a RANS dataset of the two-dimensional compressible flow over a transonic airfoil and a dataset of the surface pressure distribution over 3D wings, including shape, inflow condition, and control surface deflection variations. On the considered test cases, our approach achieves a more than three times lower test error and significantly improves generalization error on unseen geometries compared to state-of-the-art Graph Neural Network architectures. Remarkably, the method can perform inference five order of magnitude faster than the high fidelity solver on the RANS transonic airfoil dataset. Code is available at https://gitlab.isae-supaero.fr/gi.catalani/aero-nepf

==> macros.tex <==
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\esssup}{ess\,sup}
\newcommand{\DS}{D_S}
\newcommand{\weight}{w}
\DeclareMathOperator{\Tr}{Tr}

\newcommand{\barkernel}{\bar\kappa}

\newcommand{\Eone}{\textbf{E1}}
\newcommand{\Etwo}{\textbf{E2}}
\newcommand{\Ethree}{\textbf{E3}}
\newcommand{\Efour}{\textbf{E4}}

\newcommand{\kernel}{\kappa}
\newcommand{\FuncClass}{\mathbb{F}}
\newcommand{\GuncClass}{\mathbb{G}}
\newcommand{\Rade}{\mathcal{R}}
\newcommand{\Order}{\mathcal{O}}
\newcommand{\loss}{{L}}
\newcommand{\impW}{\omega}
\newcommand{\impWv}{\impW_\varepsilon}
\newcommand{\imptheta}{\theta}
\newcommand{\impthetaV}{\theta}
\newcommand{\DT}{D_T}
\newcommand{\impV}{\omega}
\newcommand{\VecOne}{\textbf{1}}
\newcommand{\FunOne}{\mathbbm{1}}
\newcommand{\Dpg}{\Delta_{p_g}}
\newcommand{\Dqg}{\Delta_{q_g}}
\newcommand{\DTg}{\Delta_{T_g}}
\newcommand{\Dpu}{\Delta_{p_u}}
\newcommand{\Dqu}{\Delta_{q_u}}
\newcommand{\DTu}{\Delta_{\T_u}}
\newcommand{\measures}{\mathcal{P}}
\newcommand{\hmax}{h_{\max}}
\newcommand{\umax}{u_{\max}}
\newcommand{\impthetamax}{\imptheta_{\max}}
\newcommand{\G}{\mathcal{G}}




\newcommand{\Comp}{\mathbb{C}}
\newcommand{\HS}{\mathcal{HS}}
\newcommand{\Hilbert}{\mathcal{H}}
\newcommand{\ttt}{\tilde{\Theta}}
\newcommand{\dinf}{d_{\infty}}
\newcommand{\tth}{\hat{\Theta}}
\newcommand{\tts}{\Theta_*}
\newcommand{\ta}{\tilde{A}}
\newcommand{\tb}{\tilde{B}}
\newcommand{\tc}{\tilde{C}}
\newcommand{\tp}{\tilde{P}}
\newcommand{\tl}{\tilde{L}}
\newcommand{\tk}{\tilde{K}}
\newcommand{\Texp}{T_{exp}}
\newcommand{\Tw}{T_{w}}
\newcommand{\Tres}{T_{reset}}
\newcommand{\alg}{\textsc{\small{GINO}}\xspace}
\newcommand{\PDE}{\textsc{\small{PDE}}\xspace}
\newcommand{\PDEs}{\textsc{\small{PDEs}}\xspace}
\newcommand{\Sys}{\textsc{\small{SysId}}\xspace}

\newcommand{\reg}{\textsc{\small{REGRET}}\xspace}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\RL}{\textsc{\small{RL}}\xspace}
\newcommand{\LQR}{\textsc{\small{LQR}}\xspace}
\newcommand{\LQG}{\textsc{\small{LQG}}\xspace}
\newcommand{\OFU}{\textsc{\small{OFU}}\xspace}


% \newcommand{\LQG}{\textsc{\small{LQG}}\xspace}
% \newcommand{\OFU}{\textsc{\small{OFU}}\xspace}
\newcommand{\FNO}{\textsc{\small{FNO}}\xspace}
\newcommand{\MDP}{\textsc{\small{MDP}}\xspace}
\newcommand{\GNO}{\textsc{\small{GNO}}\xspace}
\newcommand{\GNN}{\textsc{\small{GNN}}\xspace}
\newcommand{\FFT}{\textsc{\small{FFT}}\xspace}
\newcommand{\trpo}{\textsc{\small{TRPO}}\xspace}
\newcommand{\ppo}{\textsc{\small{PPO}}\xspace}
\newcommand{\PPO}{\textsc{\small{PPO}}\xspace}
\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}
\newcommand{\vecy}{\vec y}
\newcommand{\history}{\mathfrak{H}}
\newcommand{\trans}{T}
\newcommand{\obs}{O}
% \newcommand{\Texp}{T_{exp}}
\newcommand{\Dexp}{\mathcal{D}_{exp}}
\newcommand{\Gcl}{\mathcal{G}^{cl}}
\newcommand{\Gol}{\mathcal{G}^{ol}}

\newcommand{\TT}{\mathbb{T}}


\newcommand{\policy}{\Pi}
\newcommand{\vpi}{{\pi}}
\newcommand{\vobs}{\vec{o}}
\newcommand{\stait}{\omega}
\newcommand{\rxa}{\Gamma}
\newcommand{\rya}{\Upsilon}
\newcommand{\U}{\mathcal{U}}
\newcommand{\Est}{M_1}
\newcommand{\End}{M_2}
\newcommand{\Erd}{M_3}
\newcommand{\decompos}{\gamma}
\newcommand{\pertM}{\Delta M_3}
\newcommand{\pertMM}{\Delta \tilde{M_3}}
\newcommand{\samplenum}{m_s}
\newcommand{\reward}{\Psi}
\newcommand{\tuple}{\mathcal{M}}
\newcommand{\bellman}{\mathcal{E}}
\newcommand{\whole}{\tilde{\mathcal{M}}}
\newcommand{\approxim}{\breve{\mathcal{M}}}
\newcommand{\subst}{{\breve{\eta}}_{\vpi^*}}
\newcommand{\effect}{v}
\newcommand{\belief}{b}
\newcommand{\cost}{c}
\newcommand{\val}{J}
\newcommand{\Qfunc}{Q}

\newcommand{\block}{\Xi}
\newcommand{\vect}{Vec}
\newcommand{\rprob}{z}
\newcommand{\past}{n}
\newcommand{\OPRE}{\textsc{\small{OPRE}}\xspace}
\newcommand{\OPREIS}{\textsc{\small{OPRE-IS}}\xspace}
\newcommand{\BF}{\textsc{BF}\xspace}
% \newcommand{\IS}{\textsc{\small{IS}}\xspace}
\newcommand{\tslive}{\textsc{\small{TS-LIVE}}\xspace}
\newcommand{\olive}{\textsc{\small{OLIVE}}\xspace}
\newcommand{\cdp}{\textsc{{CDP}}\xspace}
\newcommand{\CDF}{\textsc{{CDF}}\xspace}
\newcommand{\cdps}{\textsc{{CDPs}}\xspace}
\newcommand{\ts}{\textsc{TS}\xspace}
\newcommand{\IS}{\textsc{IS}\xspace}
\newcommand{\ISClip}{\textsc{IS-Clip}\xspace}
\newcommand{\DR}{\textsc{DR}\xspace}
\newcommand{\ofu}{\textsc{OFU}\xspace}
\newcommand{\mdp}{\textsc{\small{MDP}}\xspace}
\newcommand{\pomdp}{\textsc{\small{POMDP}}\xspace}
\newcommand{\Azuma}{\mathcal{J}}
\newcommand{\Dr}{D_{\text{ratio}}}
\newcommand{\Ke}{\mathcal{K}_\epsilon}
\newcommand{\Le}{L_\epsilon}
\newcommand{\w}{W}
\newcommand{\VV}{B}
\newcommand{\vv}{b}
\newcommand{\HH}{S}
\newcommand{\hhh}{s}
\newcommand{\deltaO}{d_O}

\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt
                     \hbox{\scriptsize.}\hbox{\scriptsize.}}}%
                     =}

% Misc symbols
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Borel}{\mathbb{B}}
\newcommand{\Natural}{\mathbb{N}}
\newcommand{\calP}{\mathcal P}
\newcommand{\F}{\mathcal F}
\newcommand{\Z}{\mathcal Z}
\newcommand{\A}{\mathcal A}
\renewcommand{\P}{\mathcal P}
\newcommand{\B}{\mathcal B}
\newcommand{\X}{\mathcal X}
\newcommand{\W}{\mathcal W}
\newcommand{\T}{\mathcal T}
\newcommand{\KL}{\mathcal D_{KL}}
\newcommand{\wKL}{\wh{\mathcal{D}}_{KL}}
\newcommand{\D}{\mathcal D}
\newcommand{\Gr}{\nabla_{\theta}}
\newcommand{\Greta}{\nabla \eta}
\newcommand{\Grrho}{\nabla \rho}
\newcommand{\Grphi}{\nabla_\phi}
\newcommand{\adv}{A}
\newcommand{\TN}{N}
\newcommand{\hh}{\hat h}
\newcommand{\hL}{\hat L}
\renewcommand{\L}{\mathcal L}
\newcommand{\Hyp}{\mathcal H}
\newcommand{\Y}{\mathcal Y}
\newcommand{\V}{\mathcal V}
\newcommand{\M}{\mathcal M}
\renewcommand{\S}{\mathcal S}
\newcommand{\C}{\mathcal C}
\newcommand{\K}{\mathcal K}
\newcommand{\E}{\mathbb E}
\newcommand{\calE}{\mathcal E}
\newcommand{\cov}{\textnormal{Cov}}
%\newcommand{\V}{\mathbb V}
\newcommand{\Prob}{\mathbb P}
\newcommand{\Ind}{\mathbbm{1}}
\newcommand{\Qrob}{\mathbb Q}
\newcommand{\I}{\mathbbm 1}
\newcommand{\N}{\mathcal N}
\newcommand{\balpha}{\boldsymbol \alpha}
\newcommand{\bmu}{\boldsymbol \mu}
\newcommand{\bSigma}{\boldsymbol \Sigma}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\MV}{\textnormal{MV}}
\newcommand{\hMV}{\widehat{\textnormal{MV}}}
\newcommand{\barmu}{\bar\mu}
\newcommand{\hmu}{\hat\mu}
\newcommand{\tmu}{\tilde\mu}
\newcommand{\barvar}{\bar\sigma^2}
%\newcommand{\hvar}{\hat\sigma^2}
\newcommand{\tvar}{\tilde\sigma^2}
\newcommand{\R}{\mathfrak{R}}
\newcommand{\hR}{\widehat{\mathcal{R}}}
\newcommand{\tR}{\widetilde{\mathcal R}}
\newcommand{\Cb}{{\mtx{C}}}
%\newcommand{\var}{\sigma^2}
\newcommand{\invdelta}{1/\delta}
\newcommand{\boldR}{\mathbb R}
\newcommand{\eps}{\varepsilon}
\newcommand{\mvlcb}{\textnormal{\texttt{MV-LCB }}}
\newcommand{\clip}{\textnormal{\texttt{Clip}}}
\newcommand{\epsMonoton}{\epsilon_{\M}}
\newcommand{\ucb}{\textnormal{\textsl{UCB }}}
\newcommand{\SDF}{\textsc{\small{SDF}}\xspace}
\newcommand{\ucbv}{\textnormal{\textsl{UCB-V }}}
\newcommand{\mvlcbt}{\textnormal{\texttt{MV-LCB(t) }}}
\newcommand{\htheta}{\hat{\theta}}
\newcommand{\hi}{\hat{i}}
\newcommand{\btheta}{\bar{\theta}}
\newcommand{\tTheta}{\widetilde{\Theta}}



\newcommand{\CVaR}{\textnormal{CVaR}}
\newcommand{\VaR}{\textnormal{C}}
\newcommand{\hcvar}{\widehat{\textnormal{C}}}
\newcommand{\var}{\textnormal{V}}
\newcommand{\varXA}{\sigma^2}
\newcommand{\EXA}{G}
\newcommand{\Var}{\mathbb{V}}
\newcommand{\Cov}{\mathbb{C}}
\newcommand{\hvar}{\widehat{\textnormal{V}}}
\newcommand{\Pinit}{P_\varnothing}



\newcommand{\avg}[2]{\frac{1}{#2} \sum_{#1=1}^{#2}}
\newcommand{\hDelta}{\widehat{\Delta}}
\newcommand{\hGamma}{\widehat{\Gamma}}

\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}
\newcommand{\wb}{\overline}
 \newcommand{\mbb}{\mathbbm}
\newcommand{\cvara}{\text{CVaR}_\alpha}

% Propositions
%
%\newtheoremstyle{dotless}{}{}{\itshape}{}{\bfseries}{}{ }{}
%\theoremstyle{dotless}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{proof}{Proof}[section]
\newtheorem{proof*}{Proof}[section]
% \newtheorem{assumption}{Assumption}[section]
% \newtheorem{theorem*}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}


\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}
